Standpoint Linear Temporal Logic

Many complex scenarios require the coordination of agents possessing unique points of view and distinct semantic commitments. In response, standpoint logic (SL) was introduced in the context of knowledge integration, allowing one to reason with diverse and potentially conflicting viewpoints by means of indexed modalities. Another multi-modal logic of import is linear temporal logic (LTL) - a formalism used to express temporal properties of systems and processes, having prominence in formal methods and fields related to artificial intelligence. In this paper, we present standpoint linear temporal logic (SLTL), a new logic that combines the temporal features of LTL with the multi-perspective modelling capacity of SL. We define the logic SLTL, its syntax, and its semantics, establish its decidability and complexity, and provide a terminating tableau calculus to automate SLTL reasoning. Conveniently, this offers a clear path to extend existing LTL reasoners with practical reasoning support for temporal reasoning in multi-perspective settings.

==> translation.tex <==
	In this section, we
	%let $n$ be an arbitrary but fixed natural number and 
	present a translation $\Trans_n$ mapping any $\sltl$ formula $\phi$ to a plain $\ltl$ formula $\Trans_n(\phi)$ such that $n$-satisfiability of $\phi$ coincides with satisfiability of $\Trans_n(\phi)$.
	
	The translation	will make explicit use of a fixed, finite set $\Precsf{n}$ of precisifications with $|\Precsf{n}|=n$.

	Our translation will map any $\phi$ into a formula of (stand\-point-free) LTL. The basic idea is to ``emulate'' standpoint structures $\tuple{\Precsf{n}, \delta}$ in plain $\ltl$ structures by means of a ``superposition'' of precisifications (or state sequences), which requires to introduce $n$ ``copies'' of the original set of propositions. 
	To this end, we define our $\ltl$ vocabulary by $\mathbb{V}_{\ltl}(\Preds,\Stands,\Precsf{n})=\tuple{\Preds'}$ where $\Preds'$ contains
	\begin{itemize}
		\item for each proposition \mbox{$p\in\Preds$} and precisification \mbox{$\pr\in\Precsf{n}$}, a proposition of the form $p_\pr$. %, intuitively expressing that $p_\pr$ should capture $\interpret{\pred{P}}{\gamma(\pr)}$;
		\item for each standpoint constant \mbox{$\sts\in\Stands$} and every precisification \mbox{$\pr\in\Precsf{n}$}, a proposition of the form $\sts_\pr$, intuitively expressing that $\pr\in\lambda(\sts)$.
	\end{itemize}
	%
	The top-level translation is then defined to set\/:
	\begin{equation*}
		\Trans_n(\phi) = \textstyle\bigland_{\pr\in\Precsf{n}}\trans_n(\pr,\phi) \land \textstyle\bigland_{\pr\in\Precsf{n}}{\star}_{\pr},
	\end{equation*}

	where $\trans_n$ is inductively defined by%
	\begin{align*}
		\trans_n(\pr, p) & = p_\pr                \\
		\trans_n(\pr, \lnot\psi)                & =\lnot\trans_n(\pr,\psi)                                \\
		\trans_n(\pr, \psi_1{\,\land\,}\psi_2)  & = \trans_n(\pr,\psi_1){\,\land\,}\trans_n(\pr,\psi_2)   \\
		\trans_n(\pr, \next\psi)                & =\next\, \trans_n(\pr,\psi)                                \\
		\trans_n(\pr, \psi_1{\,\until\,}\psi_2)  & = \trans_n(\pr,\psi_1){\,\until\,}\trans_n(\pr,\psi_2)   \\
		\trans_n(\pr'\!, \standb{\ste}\psi)     & = \textstyle \bigland_{\pr\in\Precsf{n}}(\transE(\pr,\ste) \limplies \trans_n(\pr,\psi))
	\end{align*}

%
Therein, $\transE$ implements the semantics of standpoint expressions, providing for
each expression \mbox{$\ste\in\StandExps$} a propositional formula $\transE(\pr,\ste)$ over $\set{ s_\pr \guard \pr\in\Precsf{n} }$ as follows\/:%
\begin{align*}
	\transE(\pr,\sts)                  & = \sts_\pr                                        \\
	\transE(\pr,\ste_1\cup\ste_2)      & = \transE(\pr,\ste_1)\lor\transE(\pr,\ste_2)      \\
	\transE(\pr,\ste_1\cap\ste_2)      & = \transE(\pr,\ste_1)\land\transE(\pr,\ste_2)     \\
	\transE(\pr,\ste_1\setminus\ste_2) & = \transE(\pr,\ste_1)\land\neg\transE(\pr,\ste_2)
\end{align*}

%\begin{remark}
%	Note that in the first-order case the number of necessary precisifications may be infinite, thus leading to an infinite translation.
%\end{remark}
%
%\vspace{2em}

A routine inspection of the translation ensures that it can be done in polynomial time and its output is of polynomial size, provided it is applied to formulas in SSNF.


